Fast training of large kernel models with delayed projections

Classical kernel machines have historically faced significant challenges in scaling to large datasets and model sizes--a key ingredient that has driven the success of neural networks. In this paper, we present a new methodology for building kernel machines that can scale efficiently with both data size and model size. Our algorithm introduces delayed projections to Preconditioned Stochastic Gradient Descent (PSGD) allowing the training of much larger models than was previously feasible, pushing the practical limits of kernel-based learning. We validate our algorithm, EigenPro4, across multiple datasets, demonstrating drastic training speed up over the existing methods while maintaining comparable or better classification accuracy.

==> macro.tex <==
\newcommand{\EP}{EigenPro}
\newcommand{\EP1}{\EP}
\newcommand{\EP2}{\EP\,2}
\newcommand{\EP3}{\EP\,3}
\newcommand{\EP4}{\EP\,4}

==> sections/abstract.tex <==
\maketitle
\begin{abstract}


Kernel methods are well-established tools in machine learning, known for their strong theoretical foundations and versatility across a range of tasks. However, scalability has remained a key challenge, limiting their broader application. Prior work \EP{3.0} algorithm marked a significant step forward, introducing a method that  memory complexity scales linearly with model size. Yet, it is constrained by high training times, with a quadratic time complexity in model size, restricting its practical use. 

In this paper, we introduce \EP{4.0}, a novel algorithm that addresses this issue \pp{overcomes the quadratic barrier} by reducing amortized training time complexity to linear in model size. Under the same conditions as \EP{3.0}, \EP{4.0} reduces training time from several days to under an hour, while preserving performance. \EP{4.0} is the first kernel solver where amortized time complexity scales linearly with both model and training size, while memory complexity remains linear with respect to model size. We validate our method on a variety of datasets, demonstrating its advantages over previous state-of-the-art approaches. \pp{add a line about how derivation of EP4 differs from EP3}

% Kernel models have demonstrated promising outcomes across a variety of machine learning tasks. Moreover, there have been significant connections identified between  kernel methods   and deep neural networks in certain regimes. However, the problem of scaling has always been a barrier for kernel methods, limiting their applicability. Recently, the \EP{3.0} algorithm was introduced, showcasing a method to scale kernel techniques for large datasets. Nonetheless, despite the capability of \EP{3.0}  to manage large datasets, it is hindered by lengthy training times. This limitation restricts the practical use of this state-of-the-art method and does not fully address the scaling issue in real-world scenarios. In this paper, we introduce a new algorithm, \EP{4.0}, which tackles this problem. We demonstrate that it is possible to reduce the training time in the same setting as \EP{3.0} from several days to under an hour, without compromising performance. In fact, performance is maintained or even improved, surpassing all previous kernel methods in terms of training time and efficiency on large datasets. We validate these claims by testing on a variety of datasets and comparing to previous state-of-the art methods.
\end{abstract}


==> sections/distribution_shift.tex <==
\section{Distribution shift}
In this section, we show how \EP{4.0} can adapt to distribution shift. We define $\mathcal{X}_s, \mathcal{Y}_s$ as the \textit{source} distribution and $\mathcal{X}_t, \mathcal{Y}_t$ as the \textit{target} distribution. Assume we have $S$ samples from the source distribution and $T$ samples from the target distribution such that $T \ll S$.

In the following distribution as an illustration we set $\mathcal{X}_s$ to be original CIFAR-10 data set and $\mathcal{X}_t$ to be CIFAR-10C. Table \ref{tab:dist_shift} we train on 3 
\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|}
        \hline
        \textbf{Training Data} & \textbf{Accuracy (\%)} \\ \hline
        Train on Source        & 52.59                  \\ \hline
        Train on Target        & 58.4                   \\ \hline
        Train on Source + Target & 65.05                \\ \hline
    \end{tabular}
    \caption{Training Accuracies}
    \label{tab:dist_shift}
\end{table}

==> sections/expts.tex <==

\begin{algorithm}[t]
\caption{\EP4}\label{alg:eigenpro4_real}
% $(X,\y,Z,\alphavec^0,\sigma,m,s,q,\xi)$
\begin{algorithmic}[1]
\REQUIRE Data $(X,\y)$, centers $Z$, batch size $m$, Nystr\"om size $s$, preconditioner level $q,$ projection period $T$ 
%\red{should call this period instead of frequency since $T$ is in units of time. frequency would be 1/T} 
\STATE Fetch subsample $X_s\subseteq X$ of size $s$, corresponding weights $\alpha_{s}=0$
\STATE $(\Lambda,\E,\lambda_{q+1})\gets$ top-$q$ eigensystem of $K(X_s,X_s)$ 
\STATE $\D = (\Lambda^{-\!1}\!-\!\lambda_{q\!+\!1}\Lambda^{-\!2})\in\Real^{q\times q}$
\STATE $\F=\E\sqrt{\D} \in \Real^{s\times q}$
\STATE $\M\!=\! K(Z,X_s)\F\in\Real^{p\times q}$
\STATE $Z_\tmp = \emptyset$ , $\alphavec_\tmp=\emptyset$, $\alphavec_{s}=\zero_s$, $\h=\zero_p$
\WHILE{Stopping criterion is not reached}
    \FOR{$t=\{1,2,\ldots,T\}$}
\STATE Fetch minibatch $(X_m,\y_m)$
\STATE $\g_m \gets K(X_m, Z)\alphavec- \y_m$ \label{line:grad1}
\STATE $\g_m\gets\g_m +K(X_m, Z_\tmp)\alphavec_\tmp$ \label{line:grad2}
\STATE $\g_m\gets \g_m+K(X_m, X_s)\alphavec_s$ \label{line:grad3}
\STATE $Z_\tmp$.append($X_m$)
\STATE $\alphavec_\tmp$.append($ -\eta\cdot \g_m$)
\STATE $\alphavec_{s} = \alphavec_{s} +\eta\cdot \F\F\tran K(X_s,X_m)\g_m$ \label{line:update_nys_weights}
\STATE $\h \gets \h- \eta\cdot K(Z,X_m)\g_m$ 
\STATE $\h\gets\h+ \eta\cdot\M\F\tran K(X_s,X_m)\g_m$ \label{line:accumulate}\hfill %\red{better to call $\g_{acc}$ as $\h$ similar to EigenPro3}
\ENDFOR
% \STATE $\thetavec\leftarrow$ {\sf EigenPro\,2.0}$(Z,\h)$

\STATE \label{line:projection}$\thetavec\leftarrow\text{proj}_{\Zspan} (\h)$
\STATE $\alphavec\gets\alphavec- \frac{n}m\eta\thetavec$ 
\STATE $Z_\tmp \gets \emptyset$, $\alphavec_\tmp\gets \emptyset$, $\alphavec_s \gets \zero_s$, $\h\gets \zero_p$
\ENDWHILE
\end{algorithmic}
\end{algorithm}

\subsection{Improving computational efficiency}
Upon careful examination of the derivations in \eqref{eq:update}, we observe that $f_{T-1}(Z)$ have already been computed previously. This allows us to efficiently reuse $f_{T-1}(Z)$ as follows,
\begin{align}
    &f_{T-1}(Z) = K(Z,Z)\alphavec 
    - \sum_{i=1}^{T-1} K(Z,X_i)\round{ \eta (f_{i-1}(X_i) - y_i) }\nonumber \\
    &\quad + \sum_{i=1}^{T-1} K(Z,X_s) \round{ \eta \F \F\tran K(X_s,X_i) (f_{i-1}(X_i) - y_i) }\nonumber \\
    &= K(Z,Z)\alphavec 
    - \sum_{i=1}^{T-1} K(Z,X_i)\round{ \eta (f_{i-1}(X_i) - y_i) } \nonumber\\
    &\quad + \sum_{i=1}^{T-1} \eta \round{ \M \F\tran K(X_s,X_i) (f_{i-1}(X_i) - y_i) }
\label{eq:intermediate_update}
\end{align}
where $\M = K(Z,X_s)\F$. plugging this in \eqref{eq:exact_project_Z} we obtain, 

\begin{align}
    &f_{T}(Z)= K(\cdot,Z)\left(\alphavec-K^{-1}(Z,Z)\h\right), 
    \\
    &\h := -\eta\bigg( \sum_{i=1}^{T-1} 
 K(Z,X_i)\round{   (f_{i-1}(X_i) - y_i) } 
    \\&
    \phantom{:=}\quad + \sum_{i=1}^{T-1}  \round{ \M \E_q^\top K(X_s,X_i) (f_{i-1}(X_i) - y_i)} \bigg)
\end{align}

\subsection{Benefits of approximate preconditioning}
\pp{Adding this} Note that the preconditioner $\mc P^s$ allows to drastically improve the speed of the iterations. But at the same time, the Nystr\"om approximation also enables the algorithm to become tractable. Due to this approximate preconditioner, we only need to maintain $s$ temporary centers in the auxiliary model, whereas the exact preconditioner ($s=n$) makes the algorithm intractable. Theoretically we only require $s=O(\log^4 n)$ as shown in \citep{abedsoltan2023nystrom}.

\section{Numerical experiments}\label{sec:expt}




% \begin{figure*}[t]
%     \centering
% \includegraphics[width=0.8\textwidth]{figs/EP4_VS_EP3.pdf}
%     \caption{Comparison between \EP{4.0} and \EP{3.0} with number of steps and wall time.}
%     \label{fig:EP4_VS_EP3}
% \end{figure*}



\begin{figure*}[th]
        \centering 
        \begin{subfigure}{1\textwidth}
        \includegraphics[width=1.0\linewidth]{figs/ep4_ep3_epochs.png}%
        \end{subfigure}
        \begin{subfigure}{1\textwidth}
        \includegraphics[width=1.0\linewidth]{figs/legend_ep43_epochs.png}%
        \end{subfigure}
        \caption{ Multi-epoch performance and convergence comparison for \EP3 and \EP4. The detail of the experiment can be found in \Cref{appendix:expts}.
        }
    \label{fig:ep4_ep3_epochs}
\end{figure*}


% We provide evidences on different devices such as: (1) GPU:A100 (2) GPU:V100 (3) Intel(R) Xeon(R) Gold 6248 CPU.

In this section, we present evidence that our approach can perform as good as previous state of arts methods in much lower running time, up to $\times 600$ speed up on this set of experiments.  We benched mark the performance on these devices on the following data sets (1) CIFAR5M, CIFAR5M\footnote{\label{mobilenet2}feature extraction using MobileNetV2} \citep{nakkiran2020deep}, (3) ImageNet$^*$, \citep{deng2009imagenet}, (4) Webvision\footnote[2]{feature extraction using ResNet-18}, \citep{li2017webvision}, and (8) Librispeech, \citep{panayotov2015librispeech}. Details about datasets can be found in Appendix \ref{appendix:expts}. While our method is compatible with any kernel function, we opted for the Laplace kernel in our experiments due to its straightforward implementation and strong empirical performance. For handling multi-class classification, we decompose the problem into  separate binary regression tasks, where each class is predicted using targets in $\{0,1\}$. The final classification is determined by selecting the class with the maximum predicted value among all binary predictions.

\paragraph{Substantial reduction in per-epoch training time.} 
In Table \ref{tab:comparison}, we evaluate the performance and computational timing for a single epoch of our proposed model against established kernel regression methods. As noted earlier, \FALKON~ exhibits limitations due to its quadratic memory complexity. For the CIFAR5M$^*$ dataset, training with a model size of 512,000 required 1.3TB of RAM, while scaling to 1M model size necessitated over 5TB. Resource constraints limited our \FALKON~ benchmarks to model sizes of 128,000 and 64,000 for the remaining datasets. While \EP3 addresses the memory constraint, it has a significant computational overhead. \Cref{tab:comparison} shows that for model size with 1M centers, \EP4 achieves approximately $\times 500$ speedup over \EP3, averaged across multiple datasets. Notably, \EP4 maintains comparable or superior performance across all evaluated datasets relative to both baseline methods.



\paragraph{Linear time complexity with model size}
Figure \ref{fig:ep4_ep3_epochs} compares \EP4 and \EP3 across multiple training epochs, following the experimental setup established in \citet{abedsoltan_2023}. Despite \EP4 linear time complexity per iteration (compared to \EP3 quadratic complexity), it demonstrates faster convergence with fewer epochs. This efficiency gain is particularly pronounced for larger model sizes, where \EP4 maintains or exceeds \EP3 accuracy while requiring significantly fewer epochs. These results empirically validate that \EP4 algorithmic improvements translate to practical benefits: not only does each iteration run faster, but fewer iterations are needed to achieve optimal performance across diverse datasets. This empirically shows that our model has a linear time complexity with respect to the model size.


\pp{time is already mentioned in previous paragraph}

\paragraph{Linear scaling in both memory and time}  We summarize all empirical results in Figure \ref{fig:3methods} and demonstrate that our method achieves both linear memory complexity and linear time complexity (empirically verified) with respect to model size, offering the best of both worlds. For the ImageNet dataset, we trained all methods until convergence. The main limitation of \FALKON is its quadratic memory scaling with model size; in its most recent version, we were unable to run it for model sizes of 128,000 centers or larger. While \EP3 does not have the quadratic memory scaling problem, Figure \ref{fig:3methods} shows that even for a relatively small dataset like ImageNet with 1M data points, training a model size of 512,000 centers requires approximately 43 days on a single GPU to reach convergence (about 100 epochs). In contrast, our proposed model achieves convergence in approximately 3 hours, requiring only 15 epochs, with each epoch being significantly more computationally efficient than \EP3 (see Table \ref{tab:comparison}).


\begin{table*}[th]
\centering
\resizebox{\textwidth}{!}{%
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{4pt}
\footnotesize
\begin{tabular}{|c|l|cccc|}
\hline
Model size & Method & CIFAR5M*($n=5$M) & CIFAR5M ($n=6$M) & Librispeech ($n=10$M) & Webvision ($n=5.2$M) \\ \hline
\multirow{3}{*}{\centering p = 64K}
& \EP\,4 & 5m (4.6x, 88\%) & 3m (\textbf{15x}, \textbf{69\%}) & 16m (9.1x, \textbf{86.8\%}) & 2m (\textbf{45.5x}, \textbf{24.3\%}) \\
& \EP\,3 & 23m (1x, \textbf{88.3\%}) & 45m (1x, 68.8\%) & 145m (1x, 85.4\%) & 91m (1x, 24\%) \\
& Falkon & 3m (\textbf{7.67x}, 86.1\%) & 5m (9x, 57.7\%) & 9m (\textbf{16.11x}, 81.0\%) & 4m (22.75x, 21.7\%) \\ \hline
\multirow{3}{*}{\centering p = 128K}
& \EP\,4 & 5m (\textbf{10x}, 88.25\%) & 4m (\textbf{26.25x}, \textbf{70.9\%}) & 19m (\textbf{17.95x}, \textbf{87.8\%}) & 4m (\textbf{49.75x}, \textbf{24.9\%})\\
& \EP\,3 & 50m (1x, \textbf{88.42\%}) & 105m (1x, 70.3\%) & 341m (1x, 84.75\%) & 199m (1x, 24.5\%)\\
& Falkon & 9m (5.56x, 86.55\%) & 11m (9.55x, 59.4\%) & 21m (16.24x, 82.30\%) & 13m (15.31x, 22.4\%) \\ \hline
\multirow{3}{*}{\centering p = 256K}
& \EP\,4 & 7m (\textbf{18.3x}, \textbf{88.61\%}) & 6m (\textbf{130.8x}, \textbf{71.8\%}) & 24m (\textbf{120x}, \textbf{88.33\%}) & 5m (\textbf{106.2x}, \textbf{26\%})\\
& \EP\,3 & 128m (1x, \textbf{88.61\%}) & 785m (1x, 70.53\%) & $\approx$ 2 days (1x) & 531m (1x, 25.52\%) \\
& Falkon & 38m (3.37x, 86.73\%) & OOM & OOM & OOM \\ \hline
\multirow{3}{*}{\centering p = 512K}
& \EP\,4 & 12m (\textbf{44.25x}, \textbf{88.58\%}) & 10m ($>$ \textbf{288x}, 72.9\%) & 36m ($>$ \textbf{200x}, \textbf{88.89\%}) & 11m (\textbf{240x}, \textbf{27.3\%})\\
& \EP\,3 & 531m (1x, 88.56\%) & $>$ 2 days (1x) & $>$ 5 days (1x) & 2 days (1x) \\
& Falkon & 240m (2.21x, 86.71\%) & OOM & OOM & OOM  \\ \hline
\multirow{3}{*}{\centering p = 1M}
& \EP\,4 & 21m ($>$ \textbf{274x}, \textbf{88.7\%}) & 17m ($>$ \textbf{508x}, \textbf{73.8\%}) & 70m ($>$ \textbf{411x}, \textbf{89.5\%}) & 21m ($>$ \textbf{686x}, \textbf{29.3\%}) \\
& \EP\,3 & $>$ 4 days (1x) & $>$ 6 days (1x) & $>$20 days (1x) & $>$ 10 days (1x) \\
& Falkon & \textsf{OOM} & \textsf{OOM} & \textsf{OOM} & \textsf{OOM} \\ \hline
\end{tabular}
}
\caption{Comparison of \EP4, \EP3, and \FALKON~ across different model sizes and datasets after $1$ epoch. The values in parentheses represent the speedup in time over \EP3 and the resulting accuracy. Details of the experiments can be found in \Cref{appendix:expts}.\\
\pp{OOM indicates the algorithm ran out of memory. Is this CPU memory or GPU memory?}
}
\label{tab:comparison}
\end{table*}





\begin{figure}[h]
        \centering 
        \begin{subfigure}{1\textwidth}
        \includegraphics[width=0.45\linewidth]{figs/comparison_3_methods.eps}%
        \end{subfigure}
        \vspace{-20pt}
        \begin{subfigure}{1\textwidth}
        \includegraphics[width=0.5\linewidth]{figs/legend_3_methods.eps}%
        \end{subfigure}
        \caption{ Time and performance comparison for \FALKON, \EP3 and \EP4 for Imagent data set. Details of the experiments can be found in \Cref{appendix:expts}.
        \pp{Can we split this into two plots that appear below each other?}
        }
    \label{fig:3methods}
\end{figure}

% \paragraph{can be run on CPU} This 







% \begin{table*}[ht]\label{table:comparision}
% \centering
% \begin{tabular}{|c|ll|ll|ll|ll|ll|}
% \cline{1-7}
% \textbf{CPU: Xeon(R), RAM: 300G}&\multicolumn{2}{c|}{P = 16000} & \multicolumn{2}{c|}{P = 32000} & \multicolumn{2}{c|}{P = 64000} 
% \\ \cline{2-7} 
% \textbf{CIFAR5M (n = 1M)}& \multicolumn{1}{l|}{Accu.} & Time 
% & \multicolumn{1}{l|}{Accu.} & Time 
% & \multicolumn{1}{l|}{Accu.} & Time \\ \hline
% \multicolumn{1}{|c|}{\EP4} 
% & \multicolumn{1}{l|}{62.44\%} & 4007s  
% & \multicolumn{1}{l|}{64.05\%} & 4681s
% & \multicolumn{1}{l|}{65.03\%} & 6874s\\ \hline
% \end{tabular}
% \caption{We utilized the raw features from the CIFAR5M dataset. In our benchmarks, we processed a subset consisting of 1 million samples from CIFAR5M, each with dimension d = 3072, for a single epoch using \EP4. These results demonstrate that \EP4offers relatively fast performance, even when operating on a Intel(R) Xeon(R) Gold 6248 CPU.}
% \end{table*}







% \begin{table}\label{table:comparision}
% \centering
% \begin{tabular}{l|ll|ll|ll|}
% \cline{2-7}
% & \multicolumn{2}{c|}{P = 128000}   & \multicolumn{2}{c|}{P = 256000}   & \multicolumn{2}{c|}{P = 512000}    \\ \cline{2-7} 
% & \multicolumn{1}{l|}{Accu.} & Time & \multicolumn{1}{l|}{Accu.} & Time & \multicolumn{1}{l|}{Accu.} & Time  \\ \hline
% \multicolumn{1}{|l|}{EigenPro++} & \multicolumn{1}{l|}{88.2\%}     &  112.3s   & \multicolumn{1}{l|}{88.35\%}      &    198s  & \multicolumn{1}{l|}{88.36\%}     &  283s   \\ \hline
% \multicolumn{1}{|l|}{EigenPro}  & \multicolumn{1}{l|}{87.96\%}      &   1779s   & \multicolumn{1}{l|}{87.68\%}      &  4122s    & \multicolumn{1}{l|}{87.33\%}      &   13075s   \\ \hline
% \multicolumn{1}{|l|}{FALKON}    & \multicolumn{1}{l|}{86.41\%}      &   450s   & \multicolumn{1}{l|}{86.8\%}      & 2019s     & \multicolumn{1}{l|}{86.76\%}      & 14448s  \\ \hline
% \end{tabular}
% \caption{}
% \end{table}


% \begin{table}\label{table:comparision}
% \centering
% \begin{tabular}{l|ll|ll|ll|ll|ll|}
% \cline{2-11}
% &\multicolumn{2}{c|}{P = 64000} & \multicolumn{2}{c|}{P = 128000} & \multicolumn{2}{c|}{P = 256000} & \multicolumn{2}{c|}{P = 512000} &
% \multicolumn{2}{c|}{P = 1024000} \\ \cline{2-11} 
% & \multicolumn{1}{l|}{Accu.} & Time & \multicolumn{1}{l|}{Accu.} & Time & \multicolumn{1}{l|}{Accu.} & Time & \multicolumn{1}{l|}{Accu.} & Time &
% \multicolumn{1}{l|}{Accu.} & Time\\ \hline
% \multicolumn{1}{|l|}{EigenPro++} 
% & \multicolumn{1}{l|}{68.68\%} & 413s  
% & \multicolumn{1}{l|}{70.11\%} &   499s
% & \multicolumn{1}{l|}{} &
% & \multicolumn{1}{l|}{} &
% & \multicolumn{1}{l|}{} & \\ \hline
% % \multicolumn{1}{|l|}{EigenPro}
% % & \multicolumn{1}{l|}{} &  
% % & \multicolumn{1}{l|}{} &   
% % & \multicolumn{1}{l|}{} &  
% % &\multicolumn{1}{l|}{}  & 
% % & \multicolumn{1}{l|}{} & \\ \hline
% \multicolumn{1}{|l|}{FALKON}    
% & \multicolumn{1}{l|}{59.87\%} &  378s
% & \multicolumn{1}{l|}{61.12\%} &  794s
% & \multicolumn{1}{l|}{} & 
% & \multicolumn{1}{l|}{} &
% & \multicolumn{1}{l|}{} & \\ \hline
% \end{tabular}
% \caption{}
% \end{table}



%importnat tables


% \begin{table*}[ht]
% % \centering
% \hspace{-10pt}
% \label{table:comparision_cifarstar}
% \small % makes the text a bit smaller
% \begin{tabularx}{1.05\textwidth}{|c|*{10}{X|}} % using tabularx to make the table fit
% \cline{1-11}
% \thead{GPU:A100 \\ RAM:1.2T} & \multicolumn{2}{c|}{P = 64000} & \multicolumn{2}{l|}{P = 128000} & \multicolumn{2}{l|}{P = 256000} & \multicolumn{2}{l|}{P = 512000} & \multicolumn{2}{c|}{P = 1024000} \\ 
% \cline{2-11} 
% \thead{CIFAR5M*\\(n = 5M)} & \multicolumn{1}{l|}{Accu.} & Time & \multicolumn{1}{l|}{Accu.} & Time & \multicolumn{1}{l|}{Accu.} & Time & \multicolumn{1}{l|}{Accu.} & Time & \multicolumn{1}{l|}{Accu.} & Time\\ 
% \hline
% \thead{EigenPro(latest)} & \textbf{87.99\%} & 271s & 88.25\% & \textbf{309s} & 88.43\% & \textbf{406s} & \textbf{88.58\%} & \textbf{695s} & \textbf{88.74\%} & \textbf{1268s}\\ 
% \hline
% EigenPro3.0 & 88.33\% & 1359s & \textbf{88.42\%} & 3014s & \textbf{88.61\%} & 7663s & 88.56\% & 31890s & \multicolumn{2}{c|}{$>$24hrs}\\ 
% \hline
% FALKON & 86.09\% & \textbf{184s} & 86.55\% & 537s & 86.73\% & 2308s & 86.71\% & 14433s & \multicolumn{2}{c|}{out of memory}\\ 
% \hline
% \end{tabularx}
% \vspace{1pt}
% \caption{The extracted features from the pretrained 'mobilenet-2' network available in the timm library were used. The benchmarks processed the full 5 million samples of CIFAR5M for one epoch/iteration for all versions of EigenPro and FALKON. All of these experiments were run on single A100 GPU, the maximum RAM we had access to was 1.2TB which was not sufficient for FLAKON with 1M centers.}
% \end{table*}











% \begin{table*}[ht]
% % \centering
% \hspace{-18pt}
% \label{table:comparisionlibrispeach}
% \small % makes the text a bit smaller
% \begin{tabularx}{1.14\textwidth}{|c|*{11}{X|}} % using tabularx to make the table fit
% \hline
% \thead{GPU: V100 \\ RAM: 300G} & \multicolumn{2}{c|}{P = 64000} & \multicolumn{2}{c|}{P = 128000} & \multicolumn{2}{c|}{P = 256000} & \multicolumn{2}{c|}{P = 512000} & \multicolumn{2}{c|}{P = 1024000} \\ 
% \cline{2-11} 
% \thead{Librispeech* \\ (n = 10M)} & \multicolumn{1}{c|}{Accu.} & Time & \multicolumn{1}{c|}{Accu.} & Time & \multicolumn{1}{c|}{Accu.} & Time & \multicolumn{1}{c|}{Accu.} & Time & \multicolumn{1}{c|}{Accu.} & Time\\ 
% \hline
% \bf EigenPro(latest) & \multicolumn{1}{l|}{\bf86.84\%} & 980s & \multicolumn{1}{l|}{\textbf{87.80\%}} & \bf1157s & \multicolumn{1}{l|}{\bf88.33\%} & \bf1440s & \multicolumn{1}{l|}{\bf88.89\%} & \bf2185s & \multicolumn{1}{l|}{\textbf{89.49\%}} & \bf4229s\\ 
% \hline
% EigenPro3.0 & \multicolumn{1}{l|}{85.43\%} & 8697s & \multicolumn{1}{l|}{84.75\%} & 20492s & \multicolumn{2}{c|}{$>18$hrs} & \multicolumn{2}{c|}{$>24$hrs} & \multicolumn{2}{c|}{$>24$hrs}\\ 
% \hline
% FALKON & \multicolumn{1}{l|}{81.04\%} & \textbf{535s} & \multicolumn{1}{l|}{82.30\%} & 1290s & \multicolumn{2}{c|}{out of memory} & \multicolumn{2}{c|}{out of memory} & \multicolumn{2}{c|}{out of memory}\\ 
% \hline
% \end{tabularx}
% \vspace{1pt}
% \caption{The features are extracted by passing through a well-trained acoustic model (aVGG+BLSTM architecture in~\citep{hui2020evaluation} to align the length of audio and text. The task is a 301-wise classification task where different classes represent different uni-grams ~\citep{jurafsky2000speech}. The implementation of extracting features is based on the ESPnet toolkit~\citep{watanabe2018espnet}. The benchmarks processed the 10 million samples for 1 epoch/iteration for all versions of EigenPro and FALKON. All of these experiments were run on a single V100 GPU; the maximum RAM we had access to was 300GB, which was not sufficient for FALKON with more than 128K centers. ) 
% }
% \end{table*}










% \begin{table*}[ht]
% % \centering
% \hspace{-10pt}
% \label{table:comparisioncifar5m}
% \small % makes the text a bit smaller
% \begin{tabularx}{1.05\textwidth}{|c|*{10}{X|}} % 
% \hline
% \thead{GPU: V100 \\ RAM: 300G} & \multicolumn{2}{c|}{P = 64000} & \multicolumn{2}{c|}{P = 128000} & \multicolumn{2}{c|}{P = 256000} & \multicolumn{2}{c|}{P = 512000} & \multicolumn{2}{c|}{P = 1024000} \\ 
% \cline{2-11} 
% \thead{CIFAR5M \\ (n = 5M)} & \multicolumn{1}{c|}{Accu.} & Time & \multicolumn{1}{c|}{Accu.} & Time & \multicolumn{1}{c|}{Accu.} & Time & \multicolumn{1}{c|}{Accu.} & Time & \multicolumn{1}{c|}{Accu.} & Time\\ 
% \hline
% EigenPro++ & \multicolumn{1}{l|}{\bf67.62\%} & 645s & \multicolumn{1}{l|}{\textbf{68.34\%}} & \bf802s & \multicolumn{1}{l|}{\bf70.12\%} & \bf1071s & \multicolumn{1}{l|}{\bf73.10\%} & \bf1604s & \multicolumn{1}{l|}{\textbf{74.25\%}} & \bf3455s\\ 
% \hline
% FALKON & \multicolumn{1}{l|}{59.60\%} & \textbf{470s} & \multicolumn{1}{l|}{60.91\%} & 1174s & \multicolumn{2}{c|}{out of memory} & \multicolumn{2}{c|}{out of memory} & \multicolumn{2}{c|}{out of memory}\\ 
% \hline
% \end{tabularx}
% \vspace{1pt}
% \caption{The raw features of CIFAR5M were used here. The benchmarks processed the full 5 million samples of CIFAR5M with d = 3072 for one epoch/iteration for all versions of EigenPro and FALKON. All of these experiments were run on a single V100 GPU. The maximum RAM we had access to was 300GB, which was not sufficient for FALKON with 256K centers.}
% \end{table*}

==> sections/obs_design.tex <==




% \begin{figure*}
%     \centering
%     \includegraphics[clip, width=0.8\textwidth]{figs/iteration_v4.png}
%     \vskip -0.1in
%     \caption{\textbf{Overview of iteration scheme for \EP4.} The figure illustrates how the model updates are performed over multiple iterations in EigenPro4. Weights are updated using batches, and gradients are accumulated iteratively until a projection step is executed. Temporary centers and weights are maintained during auxiliary iterations, which are merged through projection after a certain number of batches. This approach reduces the computational cost by accumulating gradients before performing the projection, leading to more efficient batch processing.}
%     \label{fig:iteration_scheme}
% \end{figure*}

% \begin{figure*}
%     \centering
% \includegraphics[width=\textwidth]{figs/EP4_VS_EP3.pdf}
%     \caption{Performance and computational time comparison between \EP{4.0} \red{($T=11$)} and \EP{3.0} (equivalent to $T=1$), highlighting the impact of the projection step on the performance of \EP{4.0}. \red{which dataset is this? webvision}}
%     \label{fig:EP3_VS_EP4}
% \end{figure*}

\section{\EP\,4: algorithm design}\label{sec:highlevel}

In this section, we provide a high-level overview and illustrations to highlight the key components of \EP4 and how it significantly reduces training time.


\subsection{Flaw in \EP\,3: Overheads due to projection}

As mentioned previously, the most costly part of \EP3 is the projection phase. 






% \EP3 is a solver for training so-called \textit{General Kernel Models} which are models of the form
% \begin{align}
%     f(x)=\sum_{i=1}^p \alpha_i K(x,z_i)
% \end{align}
% The key development of \EP3 over its contemporaries was that it could train models of this form in $O(p)$ memory. This was a huge improvement over the prior state of the art which required $O(p^2)$ memory. 

\begin{table}
\centering
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{Algorithm}  
& \multicolumn{3}{c}{FLOPS}                 & \multirow{2}{*}{Memory} \\ %\cline{2-4}
& \multicolumn{1}{c}{setup} 
& \multicolumn{2}{c}{per sample} 
&
\\ \midrule
\EP{4.0} (ours)               
& \multicolumn{1}{c}{$ O(1)$}      
& \multicolumn{2}{c}{$O(p)$}              
& $O(p)$ 
\\ %\hline
\EP{3.0} 
& $ O(1)$     
& \multicolumn{2}{c}{$O(p^2)$}              
&  $O(p)$      
\\ %\hline
\FALKON            
& \multicolumn{1}{c}{$O(p^3)$}      
& \multicolumn{2}{c}{$O(p)$}              
& $O(p^2)$
\\ \bottomrule
\end{tabular}

\caption{\label{tab:computational complexity}
   \textbf{Algorithm complexity.}  with respect to number of model centers $p$. 
   Here we assumed only a constant number of epochs is needed for large scale experiments. 
   Cost of kernel evaluations and number of classes are assumed to be $O(1)$.
} 
\end{table}

However, \EP\,3 has a high cost $O(mp+p^2)$ per batch of data processed, as summarized in \Cref{tab:computational complexity}. This is especially expensive when $m\ll p$, i.e., when the batch size $m$ is  small compared to the model size $p$.

% As mentioned previously \(T\) as a crucial hyperparameter that determines the frequency of projection back to \(\Zspan\) after every \(T\) steps. Meanwhile, at every step when a new batch \((X_m, y_m)\) is fetched, it is added to a set we call ``temporary centers'' set, denoted by \(\Zt\). Starting with an empty set, \(\Zt = \emptyset\), we continuously add to \(\Zt\) with temporary centers until the step count reaches \(T\).

% Mathematically, the \EP\, algorithm is based on a stochastic projected gradient method (See \citep[Sections 4 and 5]{abedsoltan_2023} for a detailed derivation). 
% In doing so, the cost $mp$ is incurred in taking a stochastic gradient step, whereas the cost $p^2$ is the cost incurred in the projection step.

\subsection{Idea: delayed projection}

The principal distinction between \EP4 (this paper) and \EP3 involves the timing of projection back to \(\Zspan\).

% \red{I like the idea of having this quote. This quote needs to be more crisp, and perhaps go to Section 2.}
\begin{quote}
\textit{Instead of projecting back to \(\Zspan\) after each iteration, \EP4 postpones the projection for several iterations.}
\end{quote}

The key development of \EP3 over its contemporaries was that it could train models of this form in $O(p)$ memory. This was a huge improvement over the prior state of the art which required $O(p^2)$ memory.

\EP4 is a major revision to \EP3. The key improvement in \EP4 is that it amortizes the cost of projection. 

Mathematically, we take advantage of the fact that the intermediate solution between taking a gradient step and a projection can be well represented for this problem, using what we call an temporary Model, as described below in \Cref{sec:auxiliary_model}. Hence, we can \textit{delay} the projection for $T$ iterations ($T = 4$ in \Cref{fig:illustration_ep4_vs_ep3}), where $T$ is a hyperparameter with a heuristic selection method discussed in \Cref{sec:exact_computational_costs}.


Formally, the prediction function prior to the projection is no longer fixed and is now expanding. The model can be described as follows:
\begin{align}
f(x) = \underbrace{\overbrace{\sum_{\z\in Z} \alpha_{\z} K(\x,\z)}^{\text{original model}} + \overbrace{\sum_{\z\in Z_{\tmp}} \beta_{\z} K(\x,\z)}^{\text{temporary model}}}_{\text{auxiliary model}}
\end{align}
where $\alpha_{\z}$ refers to the weights corresponding to the original model center $\z$ and $\beta_{\z}$ refers to the weights corresponding to the auxiliary model center. 

The following Figure \Cref{fig:illustration_ep4_vs_ep3} illustrate this mechanism, see \Cref{sec:exact_computational_costs} for a detailed analysis of cost amortization.

\begin{figure}[h]
    \centering
    \includegraphics[clip, trim=6cm 9cm 6cm 9cm, width=0.5\textwidth]{figs/eigenpro4_batching.pdf}
    \caption{\textbf{Design of EigenPro4.} An illustration of how batches of data are processed by the two algorithms. EigenPro3 involves an expensive  \textit{projection} step when processing every batch of data. EigenPro4 waits for multiple batches to be processed before running the projection step for all of them together. This reduces the amortized cost for processing each batch.}
    \label{fig:illustration_ep4_vs_ep3}
\end{figure}



\begin{figure*}[!ht]
    \centering
\includegraphics[width=1.0\textwidth]{figs/EP4_VS_EP3.pdf}
    \caption{Performance and computational time comparison between \EP{4.0} ($T=11$) and \EP{3.0} (equivalent to $T=1$), highlighting the impact of the projection step on the performance of \EP{4.0}. The detail of the experiment can be found in \Cref{appendix:expts}.}
    \label{fig:EP3_VS_EP4}
\end{figure*}


In fact, \EP3 is a special case of \EP4 with parameter $T=1$. However, we show in \cref{eq:optimal_T} that to minimize total time of training, the optimal value of $T$ is in fact proportional to $\frac{p}{m}.$ For this value of $T$, the cost of training per batch is $O(p)$.


Figure~\ref{fig:EP3_VS_EP4} compares the performance of EP4 and EP3 across iteration steps. EP4's accuracy improves as it expands by incorporating temporary centers, then drops after each projection back to the original centers. This drop aligns EP4's performance with that of EP3, which projects back at every step. The left panel of Figure~\ref{fig:EP3_VS_EP4} shows that both methods achieve similar accuracy, while the right panel demonstrates that EP4 runs significantly faster than EP3. As training continues, the accuracy loss from each projection in EP4 progressively diminishes.

% \subsection{Compatible with streaming data}
% \EP{} family of algorithms does batching. FALKON does not take advantage of batching.\amir{this is not correct in principle they can also make theri algorithm batch freindly.}







% \subsection{Auxiliary model at intermediate steps}



% \label{sec:auxiliary_model}
% In \EP4 we introduce the notion of an auxiliary and temporary model. For each step $t$, \EP4 defines a new model of the form


% \begin{align}
%     f_t(x)&=f_{kT}(x) + \wt f_t(x),\quad kT<t < (K+1)T
% \end{align}
% which is the sum of the original model $f_{kT}$ trained till $kT$ iterations, and an auxiliary  model created from $\wt p_t=m(t-kT-1)$ temporary centers $\set{\wt z_i}_{i=1}^{\wt p_t}$. The temporary model is defined as
% \begin{align}
%     \wt f_t(x)&=\sum_{j=1}^{\wt p_t} \wt\alpha_i K(x,\wt z_i)
%     % \\
%     % &:= \wt f_{t-1}(x) +  K(x, X_{t-1})\wt\alphavec_{t-1}\label{eq:temp_model_iterative}
% \end{align}

% The weights $\wt\alphavec_{i}$ are computed according to the procedure detailed in Section~\ref{sec:derivation}. At each step $t$, new temporary centers $\set{\wt z_i}_{i=\wt p_t}^{\wt p{t+1}}$ are incorporated into the auxiliary model, where these temporary centers correspond to the processed batch at each iteration. The temporary model expands incrementally before each projection step, after which it is projected back onto the original centers.



% Figure~\ref{fig:EP3_VS_EP4} compares EP4 and EP3 performance over iteration step. EP4's accuracy grows as it adds temporary centers, then drops when projecting back to the original centers. However, this drop is make the perforamcne of EP4 comparabel to  EP3, which projects back at every step. The right panel of Figure~\ref{fig:EP3_VS_EP4} shows that EP4 runs much faster than EP3 and left panel shows the performance maintain the same. As training continues, the accuracy drops after each projection diminishes.

% where $X_{t-1}$ is the previous 
% Here $\wt\alphavec_{i}$ are weights calculated appropriately, as explained later in \Cref{sec:derivation}. At step $t$, the temporary centers $\set{\wt z_i}_{i=\wt p_t}^{\wt p_{t+1}}$ are added to the auxiliary model, in fact temporary cneters are the proccesed batch at each iteration. 

% Therefore, after each step prior to projection step the temporary model expands and eventully at the the projection step it will be projected back to the original centers. \Cref{fig:EP3_VS_EP4} compares the perforamcne evlution between \EP4 and \EP3, as it can be seen the model perforamnce improves as the model is expanding with temporatry centers and after the projection step we see a drop in the perforamnce due to the information loss during the projection. However, this information loss is no greater that \EP3 where we project back to the original model space for each iteration. Due to this delayed projection the right panel of \Cref{fig:EP3_VS_EP4} shows drastci speead up without compromising the performance. Moreover it is evident that as we proggress the trainig this drop in perfroamcne after each iteration diminshes.
% These temporary centers consist of training inputs processed in that step.

% For each step, the auxiliary model $f_t$ is used to calculate the gradients. These gradients are accumulated over $T$ iterations,
% % at the end of which a projection step is performed to obtain $f_{(k+1)T}$ from $F_{(k+1)T}$.
% after which, \EP4 performs the same \textit{Projection} step as \EP3, see Figure \ref{fig:illustration_ep4_vs_ep3} for visual illustration. 
% This is a form of model order reduction\amir{any citation?} to obtain $f_{(k+1)T}$ from $F_{(k+1)T}$.



% \begin{figure}[h]
%         \centering 
%         \begin{subfigure}{1\textwidth}
%         \includegraphics[width=0.5\linewidth]{figs/comparison_3_methods.eps}%
%         \end{subfigure}
%         \vspace{-20pt}
%         \begin{subfigure}{1\textwidth}
%         \includegraphics[width=0.5\linewidth]{figs/legend_3_methods.eps}%
%         \end{subfigure}
%     \caption{Performance and computational time comparison between \EP{4.0} \red{($T=11$)} and \EP{3.0} (equivalent to $T=1$), highlighting the impact of the projection step on the performance of \EP{4.0}. \red{which dataset is this? webvision}}
%     \label{fig:EP3_VS_EP4}
% \end{figure}




% \subsection{Projection}

% The projection step line \ref{line:projection} in \Cref{alg:eigenpro4_real} approximately solves the linear system of equations
% \begin{align}\label{eq:projection_linear_system}
%     K(Z,Z)\thetavec=\wt f_{(k+1)T}(Z)
% \end{align}
% where $K(Z,Z)$ is the $p\times p$ kernel matrix of pairwise evaluations of the kernel function over the model centers $Z$. Furthermore, the RHS $\wt f_{(k+1)T}(Z)$ is the evaluation of the temporary model at the model centers.
% The linear system of equations in \eqref{eq:projection_linear_system} is solved approximately using the \EP2 algorithm which costs $O(p^2)$ flops and $O(p)$ memory.

% % using $T_{\sf ep2}$ epochs of the \EP2 algorithm. This step requires $p^2 \cdot T_{\sf ep2}$ FLOPS.

% Note that for an efficient implementation, we obtain $\wt f_{(k+1)T}(Z)\in\Real^p$ iteratively as follows, 
% \begin{align*}
% \wt f_{t}(Z)=\wt f_{t-1}(Z) + \sum_{i=\wt p_{t-1}}^{\wt p_t}\wt\alpha_i K(Z,\wt z_i).
% \end{align*}
% The quantities $K(Z,\wt z_i)\in\Real^p$ are re-used in the above computation, they were used to obtain the gradient at step $t$.

% \subsection{Compatibility with preconditioning}
% To speed up iterations we apply spectral preconditioning similar to \citep{ma2019kernel,abedsoltan_2023}. The preconditioning comes at a negligible additional cost but has huge benefits to the convergence speed. The Nystr\"om approximate preconditioner \citep{abedsoltan2023nystrom} plays well with our scheme above. Adding preconditioning means we need to account for $s=O(\log^4n)$ additional temporary centers in our auxiliary model.


==> sections/obs_intro.tex <==
\section{Introduction}

Kernel methods~\citep{scholkopf2002learning,shawe2004kernel} are foundational in machine learning, recognized for their strong theoretical basis and wide applicability. They have served as the foundation for understanding many significant phenomena in modern machine learning~\citep{jacot2018neural,belkin2018understand,belkin2019reconciling,zhang2021understanding}. Additionally, kernel methods are widely applied in fields such as bioinformatics, robotics, and finance~\citep{scholkopf2004kernel,kocijan2016modelling,dixon2020machine}.
Despite the scaling of large transformers to trillions of parameters and data points, achieving scalability for classic kernel methods remains surprisingly challenging. In this paper, we propose a new method, \EP4, to address these challenges and achieve unprecedented scalability for kernel methods in both theoretical complexity and practical efficiency.
By utilizing preconditioned stochastic gradient iterations, \EP4 integrates seamlessly with modern training infrastructure, resulting in high resource utilization and a minimal number of epochs required for convergence.


\begin{table}[h]
    \centering
    \begin{tabular}{|p{1.5cm}|p{6cm}|}
        \hline
        \textbf{Method} & \textbf{Requirements} \\ \hline
        Direct solve & Very high flops and memory: quadratic to cubic in data / model size \\ \hline
        Conjugate gradient & High setup cost: quadratic in model size; needs double precision \\ \hline
        Stochastic gradient & Costly iteration when model centers differ from data \\ \hline
    \end{tabular}
    \caption{Summary of existing kernel methods and their requirements.}
    \label{tab:methods_requirements}
\end{table}

In a regression setting, training a kernel machine is equivalent to solve the corresponding kernel matrix inversion problem. A direct method to solve such a problem with $n$ samples requires $O(n^3)$ flops computation and often $O(n^2)$ memory. Thus, the cost of the direct method grows rapidly, making it intractable for datasets with more than $\sim10^5$ data points.

To address this challenge, various methods employing iterative algorithms and approximations have been proposed. Among these, Gradient Descent (GD)-based algorithms like Pegasos~\citep{shalev2007pegasos} and \EP~\citep{ma2017diving,ma2019kernel} have significantly reduced the computational complexity to $O(n^2)$. These methods, adaptable for stochastic settings, offer more efficient implementations. Nevertheless, the scalability of kernel machines remains constrained by the inherent linkage between the model size and the training set.

Furthermore, the Nystr\"om methods have emerged as a favored approach for scaling kernel machines, with seminal works with~\citep{williams2000using} paving the way. Methods such as {\NYTRO}~\citep{camoriano2016nytro} and {\FALKON}~\citep{rudi2017falkon} leverage the Nystr\"om Approximation (NA) in combination with other strategies to enhance performance. {\NYTRO} merges NA with gradient descent to improve condition number, whereas FALKON combines it with the Conjugate Gradient method, facilitating the handling of large training sets. However, these strategies are limited by model size due to memory restrictions, exhibiting quadratic scaling in relation to the size of the model. For instance, scaling FALKON~\citep{meanti2020kernel} method to a model size of $512,000$ necessitates over 1TB of RAM, surpassing the capacity of most high-end servers available today.

\begin{table}[h]
\centering
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{Algorithm}  
& \multicolumn{3}{c}{FLOPS}                 & \multirow{2}{*}{Memory} \\ %\cline{2-4}
& \multicolumn{1}{c}{setup} 
& \multicolumn{2}{c}{per sample} 
&
\\ \midrule
\EP4 (ours)               
& \multicolumn{1}{c}{$\wt O(1)$}      
& \multicolumn{2}{c}{$O(p)$}              
& $O(p)$ 
\\ %\hline
\EP3 
& $\wt O(1)$     
& \multicolumn{2}{c}{$O(p^2)$}              
&  $O(p)$      
\\ %\hline
\FALKON            
& \multicolumn{1}{c}{$O(p^3)$}      
& \multicolumn{2}{c}{$O(p)$}              
& $O(p^2)$
\\ \bottomrule
\end{tabular}

\caption{\label{tab:computational complexity}
   \textbf{Algorithm complexity.}  with respect to number of model centers $p$. 
   Here we assumed only a constant number of epochs of \EP{2.0} is needed for large scale experiments. 
   Cost of kernel evaluations and number of classes are assumed to be $O(1)$.
} 
\end{table}


Recently, \EP3 was introduced in~\citep{abedsoltan_2023}. Unlike previous versions, \EP3 distangle the model from the training set, similar to FALKON, but with the added advantage that its memory requirements scale linearly with the model size. This advancement makes it feasible to tackle kernel models of sizes previously deemed unattainable. However, its time complexity remains quadratic relative to the model size, significantly slowing its practical application. 

% For instance, running a single epoch on 10 million data points for a model size of 512,000 necessitates over a day of training on a single GPU, severely limiting the practicality of employing \EP{3.0}.


In this paper, we build upon \EP3 and introduce \EP4. This new algorithm retains the advantageous features of \EP3, such as decoupling the model from the training set and linear scaling in memory complexity. Moreover, it significantly improves upon the time complexity, achieving amortized linear scaling in model size without compromising performance. 


\subsection{Main contribution}


% We introduce a kernel regression solver with linear amortized time complexity per iteration, which scales linearly with both the number of training samples and the model size, while maintaining linear memory complexity with respect to the model size. Crucially, this scaling is achieved without any loss in performance. For instance, a single epoch on 10 million data points with a model size of 512,000 can now be completed in about half an hour, offering nearly a 50× speed-up compared to state-of-the-art kernel solvers, all while maintaining superior generalization performance.

We introduce a kernel regression solver with per-iteration complexity that scales linearly in both model size and data size, while also converging in fewer epochs. To our best knowledge, \EP4 is the {\bf first} kernel method to achieve this linear scaling alongside near-optimal convergence rates in practice.
This characteristic enables orders of magnitude speedup over state-of-the-art kernel methods, especially at large scales, making the training of very large kernel models feasible. For instance, with \EP4, a single epoch on a dataset containing 10 million data points with a model of 1 million centers can be completed in around 70 minuets — providing more than \textbf{400×} speed-up over state-of-the-art kernel solvers. Despite the efficiency, \EP4 maintains superior generalization performance compared to current methods.

\begin{figure}[h]
    \centering
\includegraphics[width=0.4\textwidth]{figs/Time_comparison_with_performance.pdf}
    \caption{Per epoch time comparison between different solvers. The testing accuracy of each step is also reported.}
    \label{fig:EP4_VS_EP3}
\end{figure}



\begin{algorithm}[th]
\caption{\EP4}\label{alg:eigenpro4_real}
% $(X,\y,Z,\alphavec^0,\sigma,m,s,q,\xi)$
\begin{algorithmic}[1]
\REQUIRE Data $(X,\y)$, centers $Z$, batch size $m$, Nystr\"om size $s$, preconditioner level $q,$ projection period $T$ 
%\red{should call this period instead of frequency since $T$ is in units of time. frequency would be 1/T} 
\STATE Fetch subsample $X_s\subseteq X$ of size $s$, corresponding weights $\alpha_{s}=0$
\STATE $(\Lambda,\E,\lambda_{q+1})\gets$ top-$q$ eigensystem of $K(X_s,X_s)$ 
\STATE $\D = (\Lambda^{-\!1}\!-\!\lambda_{q\!+\!1}\Lambda^{-\!2})\in\Real^{q\times q}$
\STATE $\F=\E\sqrt{\D} \in \Real^{s\times q}$
\STATE $\M\!=\! K(Z,X_s)\F\in\Real^{p\times q}$
\STATE $Z_\tmp = \emptyset$ , $\alphavec_\tmp=\emptyset$, $\alphavec_{s}=\zero_s$, $\h=\zero_p$
\WHILE{Stopping criterion is not reached}
    \FOR{$t=\{1,2,\ldots,T\}$}
\STATE Fetch minibatch $(X_m,\y_m)$
\STATE $\g_m \gets K(X_m, Z)\alphavec- \y_m$ \label{line:grad1}
\STATE $\g_m\gets\g_m +K(X_m, Z_\tmp)\alphavec_\tmp$ \label{line:grad2}
\STATE $\g_m\gets \g_m+K(X_m, X_s)\alphavec_s$ \label{line:grad3}
\STATE $Z_\tmp$.append($X_m$)
\STATE $\alphavec_\tmp$.append($ -\eta\cdot \g_m$)
\STATE $\alphavec_{s} = \alphavec_{s} +\eta\cdot \F\F\tran K(X_s,X_m)\g_m$ \label{line:update_nys_weights}
\STATE $\h \gets \h- \eta\cdot K(Z,X_m)\g_m$ 
\STATE $\h\gets\h+ \eta\cdot\M\F\tran K(X_s,X_m)\g_m$ \label{line:accumulate}\hfill %\red{better to call $\g_{acc}$ as $\h$ similar to EigenPro3}
\ENDFOR
% \STATE $\thetavec\leftarrow$ {\sf EigenPro\,2.0}$(Z,\h)$

\STATE \label{line:projection}$\thetavec\leftarrow\text{proj}_{\Zspan} (\h)$
\STATE $\alphavec\gets\alphavec- \frac{n}m\eta\thetavec$ 
\STATE $Z_\tmp \gets \emptyset$, $\alphavec_\tmp\gets \emptyset$, $\alphavec_s \gets \zero_s$, $\h\gets \zero_p$
\ENDWHILE
\end{algorithmic}
\end{algorithm}

% We introduce, to the best of our knowledge, the first kernel regression solver whose time complexity scales linearly with both the number of training samples and the model size, while memory complexity remains linear with respect to model size. Importantly, this scaling is achieved without sacrificing performance. As an example, running a single epoch on 10 million data points with a model size of 512,000 can now be completed in approximately half an hour; almost $\times50$ times speed up compare to~\EP{3.0}\citep{abedsoltan2023toward}.
% The summary of time and memory complexity of our method with previous state-of-the art method can be found in table \Cref{tab:computational complexity}.





% \subsection{Motivation and Impact}

% This 


==> sections/online.tex <==
\section{Online Learning and Center Selection}

Online learning is the dominant learning paradigm for many important industry applications such as advertising, recommendation, and fraud detection.
It makes the model robust against covariate shift, which occurs when the input data distribution changes over time, by incrementally taking into account new data when they become available.
This adaptability allows the model to remain accurate and relevant in dynamic production environments.
Moreover, online learning enables real-time personalization and rapid adaptation to changing user preferences.
Since such robustness and flexibility are critical for production systems, the business decision for adopting a modeling approach typically relies heavily on whether this approach is capable of online learning, as it directly impacts the user experience and the performance of the production system.

The proposed \EP{4.0} is the first kernel method that allows for practical online learning at large scale with negligible overhead.

Recall that with centers $Z_t = \{z_{t,1}, \ldots, z_{t,d}\}$ and corresponding weights $W_t = \{w_{t,1}, \ldots, w_{t,d}\}$, the model makes prediction on input data $x$ by\\
\[
f_t(x) = \sum_{i=1}^d k(z_{t,i}, x) w_{t,i}
\] 
We then outline an online version of EigenPro below:

% \begin{table}[h!]
% \centering
% \begin{tabular}{|p{14cm}|}
% \hline
% \vspace{-0.2em}
% \textbf{Hyperparameters} \\
% \vspace{-0.5em}
% \begin{itemize}
%     \item Projection criteria
%     \item Center selection method $h$
%     \item Projection method $\pi$
% \end{itemize} \\
% \hline
% \vspace{-0.2em}
% \textbf{At iteration $t$:} \\
% \vspace{-0.5em}
% \begin{enumerate}
%     \item Obtains streaming data $(X_t, Y_t)$ where $X_t = \{x_{t,1}, \ldots, x_{t,m}\}$ is a mini-batch of size $m$.
%     \item Adds temporary centers $Z' = Z_t' \cup X_t$ and add corresponding weights to $W'$.
%     \item If the projection criteria are met:
%     \begin{enumerate}
%         \item Adds all current centers and temporary centers as candidate centers $Z_c = Z_t \cup Z'$.
%         \item Adds more candidate centers such as k-means centers to $Z_c$ if needed.
%         \item Selects centers $Z_{t+1} = h(Z_c, W_t, W')$. The selection procedure might need to access the previous training data.
%         \item Obtains the corresponding weights by projection $W_{t+1} = \pi(Z_t \cup Z', W_t \cup W', Z_{t+1})$
%     \end{enumerate}
%     \item Else, $Z_{t+1} = Z_t$.
% \end{enumerate} \\
% \hline
% \end{tabular}
% \caption{Online Learning with EigenPro}
% \end{table}


\begin{algorithm}[t]
\caption{Online Learning with EigenPro}\label{alg:online_eigenpro}
\begin{algorithmic}[1]
\Require Projection criteria, center selection method $h$, projection method $\pi$
\State Initialize centers $Z$, weights $W$
\While{Stopping criterion is not reached}
    \State Fetch streaming data $(X_t, Y_t)$ where $X_t = \{x_{t,1}, \ldots, x_{t,m}\}$ is a mini-batch of size $m$
    \State Add temporary centers $Z' = Z \cup X_t$ and corresponding weights to $W'$
    \If {Projection criteria are met}
        \State Add all current centers and temporary centers as candidate centers $Z_c = Z \cup Z'$
        \State Add more candidate centers such as k-means centers to $Z_c$ if needed
        \State Select centers $Z_{t+1} = h(Z_c, W, W')$. The selection procedure might need to access the previous training data
        \State Obtain the corresponding weights by projection $W_{t+1} = \pi(Z \cup Z', W \cup W', Z_{t+1})$
    \Else
        \State $Z_{t+1} = Z$
    \EndIf
    \State Update $Z \gets Z_{t+1}$, $W \gets W_{t+1}$
\EndWhile
\end{algorithmic}
\end{algorithm}


==> sections/software.tex <==
\section{Software implementation overview}

\red{description of abstractions}

\red{example code. Example. not accurate}

\begin{lstlisting}
from eigenpro import EigenPro4Optimizer
X, y = SOME_DATASET
Z = SOME_CENTERS # eg X[randint(0, n, p)]
n, d = X.shape()
n, c = y.shape()
p, d = Z.shape()

K = LaplacianKernel(bandwidth=1.0)
model = KernelModel(
    kernel=K, 
    centers=Z
)

optimizer = EigenPro4Optimizer(
    model, 
    projection_interval=T
)

model.train()
for _ in range(epochs):
    for (Xm, ym) in dataloader:
        EigenPro4(model, Xm, ym)

print(f"Model trained for {epochs} epochs")
\end{lstlisting}
